Descriptor: LYNRED Mobility Dataset Multimodal Detection Subset (LYNRED-MDS)

Current road safety systems primarily focus on minimizing post-collision damage. However, advances in algorithmic perception are shifting focus toward early collision prediction, especially in lowvisibility conditions like nighttime or fog, where thermal infrared sensing outperforms both human vision and RGB imaging. While available RGB-infrared datasets such as FLIR ADAS and LLVIP are good benchmarks, they mostly consist of clear weather and overly simple scenarios. In this article, we introduce the LYNRED-MDS: Multimodal Detection Subset, a subset of the LYNRED Mobility Dataset, comprised of 4000 RGB-infrared image pairs captured under diverse weather, lighting, and road conditions around Grenoble, France. Our dataset spans varied driving contexts (urban, rural, mountainous, etc.) and a vehicle fleet compliant with Western European standards. Thermal cross-dataset evaluation using a YOLOv8n baseline suggests that our dataset offers strong generalization potential for pedestrian detection in driving scenarios. By covering critical edge cases, our dataset supports the development of more reliable and deployable vision systems for advanced driver-assistance systems.

==> Parts/00_intro.tex <==

Recent advancements in technology have triggered a significant shift in regulatory frameworks designed to enhance the safety of vulnerable road users (VRUs). These frameworks increasingly focus on the integration of advanced technologies, particularly in the realm of vehicle safety systems. With technologies such as computer vision-based pedestrian and cyclist detection systems proving effective in reducing VRU-related collisions~\cite{tomtom, NHTSA, EUGSR}, many jurisdictions now require the inclusion of advanced driver assistance systems (ADAS) in new vehicles. For example, the European Union's General Safety Regulation now requires features like automated emergency braking tailored for VRU scenarios~\cite{EUGSR}, and organizations like the European New Car Assessment Programme have incorporated these systems into their vehicle safety assessment protocols~\cite{tomtom}. In the United States, the National Highway Traffic Safety Administration similarly emphasizes on adopting ADAS technologies, in particular for Automatic Emergency Breaking (AEB) systems~\cite{NHTSA}. In that regard, they impose to these AEB systems to avoid impact at 62mph (about 100km/h). This means emergency breaking systems should be able to detect objects, in this case human beings, at about 60m if we suppose an AEB reaction time to be close to instantaneous. \\


\begin{figure*}
   
   \centering
   \includegraphics[width=0.32\textwidth]{images/image(8).png}
   \hfill
   \includegraphics[width=0.32\textwidth]{images/statue_nuit.png}%
   \hfill
   \includegraphics[width=0.32\textwidth]{images/skieur.png}
  \caption{Three samples of the multimodal detection subset of the LYNRED mobility dataset showing the diversity of the dataset.}\label{label}
  \label{fig:Extracts}
\end{figure*}


In addition to vehicle-based systems, regulatory efforts have extended to urban infrastructure. Many cities have introduced mandates for adaptive traffic controls, smart crosswalks, and reduced speed limits in high--density VRU zones~\cite{EUGSR}. These efforts build on traditional safety measures---such as crash worthiness standards and pedestrian--friendly design,---but also reflect a broader shift toward leveraging cutting-edge technologies like computer vision and smart sensors to address VRU safety in a more comprehensive manner. This shift toward predictive safety has been facilitated by advancements in computer vision and sensor technologies, which have both reduced the cost of sensors and improved the robustness of detection systems over the last decades. The automotive industry has, since then,  embraced these technologies. \\

The publication of public datasets sparked further research in the field. Notable among these are the Kitti~\cite{Geiger2012CVPR} and Cityscapes~\cite{Cordts2016Cityscapes} datasets, which introduced demanding tasks such as semantic segmentation and depth estimation, mostly leveraging light detection and ranging (LiDAR) data. Alongside those active sensor technologies, several thermal imaging datasets have made their ways in the in the pedestrian or VRU detection community, demonstrating the efficiency of passive IR imaging under various lighting conditions. Indeed, Long wave Infrared (LWIR) or thermal sensors---unlike visible light or RGB sensors---do neither rely on external light sources such as the sun or a car's headlights, nor on emitted signals like LiDAR or ultrasound sensors. Indeed, infrared imaging uniquely relies on thermal radiation of the objects, \idest the quantity of photons released by a corpse as a function of its temperature~\cite{corsi2015new}. This makes it an ideal candidate for pedestrian detection tasks. As a matter of fact, humans have an internal temperature of 36.6\si{\celsius}~\cite{ley2023defining} and hence tend to be easily distinguishable from their environment~\cite{gonzalez2016pedestrian,dona2024thermal}.\\

The collection of visible data being relatively inexpensive, those IR datasets often go paired with visible RGB sensor data. Most modern vehicles are actually already equipped with a standard optical camera. As a result, RGB-T (visible-thermal) or  RGB-T (visible-infrared) datasets have been released. The first work on those paired visible and thermal images in object detection was through datasets such as KAIST multi-spectral~\cite{hwang2015multispectral} and CVC-14~\cite{gonzalez2016pedestrian}. The KAIST multispectral dataset has been particularly influential in the development of VRU detection tasks. Following KAIST, the FLIR thermal ADAS dataset~\cite{FLIR} helped further establish the utility of thermal-visible pairs for driving scenarios~\cite{wilson2023recent}. It succeeded in raising awareness for VRU detection and paved the way for this new paradigm~\cite{wilson2023recent}. In addition to the on--vehicle datasets, more recent static datasets like LLVIP~\cite{jia2021llvip} have been published. Although they differ from the original focus on  RGB-T object detection for on--vehicle scenarios, they provide valuable insights for research in  RGB-T object detection. Additionally, some datasets have introduced new tasks for infrared modalities, such as depth estimation alongside object detection~\cite{franchi2024infraparis}.\\

Despite the extensive literature on thermal datasets, most of the existing datasets focus on favorable detection scenarios, primarily---if not, exclusively,---using ideal weather conditions for both thermal and visible modalities. Extreme weather conditions and challenging real--world environments are rarely present. Yet, the systems developed using these datasets are expected to perform well, even under these situations. To address this gap, we present here a recently published RGB-T object detection dataset: the multimodal detection subset of the LYNRED Mobility Dataset (LYNRED-MD). The latter offers images acquired during more diverse and realistic driving scenarios. A few snapshot pairs are presented in Figure~\ref{fig:Extracts}. 

==> Parts/01_Realted.tex <==
\section{Related datasets}
\label{sec:related}

In this section, we present the current state of the art datasets, their specifications and assess their contribution to the literature. A summary can be found in Table~\ref{tab:datasetsspecs}.


\paragraph{KAIST Multi-spectral}

Published in 2015 by The Korean Advanced Institute of Science and Technologies, it includes over 95k aligned color-thermal pairs of images and 103,128 annotations in its first version \cite{hwang2015multispectral}. The history of the dataset as described by \cite{zhang2020multispectral} is that original labels were first criticized by \cite{liu2016multispectral} who chose to only use a subset of all the provided images. Then \cite{li2018multispectral} proposed a sanitized version of this dataset, correcting the original annotations that were highly imprecise. Despite its relatively low resolution by today’s standards, the cleaned version remains widely used for model evaluation and comparison.

\paragraph{FLIR thermal ADAS}

Proposed by Teledyne FLIR, it is an Advanced Driving Assistant System data base. Its second version is composed of 13k pairs of  RGB-T images, offered both in 16 and 8bit for the infrared images. Initially annotated with 5 classes, it was extended to 16 classes with the release of its second version in 2022~\cite{FLIR}. It presents images acquired mostly in perfect weather conditions, where neither the visible nor the infrared sensors are significantly challenged. The dataset was criticised by~\cite{zhang2020multispectral} for offering unaligned annotations for the RGB and infrared modalities. The mislabelled images were eventually removed, leading to the FLIR aligned subset of the original FLIR ADAS dataset.


\paragraph{LLVIP}

Although it consists only of static video surveillance images, the LLVIP dataset~\cite{jia2021llvip} is an other recent dataset that caught community's interest thanks to its size and the quality of its images and labels. It makes a good benchmark for multispectral object detection models. Furthermore, the used camera setup offers optically aligned infrared and visible images, hence removing the geometrical alignment constraint that most other datasets of its kind suffers from. This explains the growing attention this dataset has gotten since its release in 2021.

\paragraph{M3FD}
Proposed by Liu \etal~\cite{m3fd}, it consists of both static and on-vehicle images captured in Dalian, China. This dataset offers 4.2k  RGB-T pairs for training and 300 for testing, and  6 annotated classes (People, Car, Bus, Motorcycle, Lamp, Truck) representing most road users. Even though it is on the smaller side of the spectrum for  RGB-T datasets, the diversity of scenes offered, as well as the associated annotations on weather conditions and light conditions make it an interesting case study for real-world ADAS scenarios. In addition to the original annotations, \cite{Deevi_2024_WACV} offers further labels for weather conditions that can be useful for evaluation purposes.


\begin{table*}[!htbp]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{lrcccccccccc}
            \hline
             %\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}

            \multicolumn{3}{c}{} & \multicolumn{2}{c}{Camera setup} & \multicolumn{2}{c}{\makecell{Image resolution \\ (Width $\times$ Height)}} & \multicolumn{2}{c}{\makecell{Intermodal \\
                Alignment}} & \multicolumn{3}{c}{\makecell{Metadata}}   \\ 
            
            \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
            
            Datasets &  \makecell[c]{\# train \\ image pairs } &  \# classes &  On vehicle &  Stationary &  IR &  RGB &  Fully Aligned &  Chessboard &  \makecell{Outside\\temperature} &  Season &  Occlusion \\ 
            
            
            \hline%\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
            
            KAIST sanitized \cite{chen2024amfd} & \num{47.5}k  & 1 & \checkmark & — & 640 $\times$ 480 & 640 $\times$ 480 & \checkmark & — & — & — & \checkmark \\ 
            FLIR ADAS \cite{FLIR} & 13k\phantom{.0} & 16 & \checkmark & — & 640 $\times$ 512 & 1800 $\times$ 160 $^\star$ & — & \checkmark & — & — & \checkmark \\  
            LLVIP \cite{jia2021llvip} & 15k\phantom{.0} & 1 & — & \checkmark & 1080 $\times$ 720 & 1080 $\times$ 720 &\checkmark & — & — & — & —  \\ 
            M3FD \cite{m3fd} & \num{4.2}k\phantom{.0} & 6 & \checkmark & \checkmark & 1024 $\times$ 768 $^\star$ & 1024 $\times$ 768 $^\star$ & \checkmark & — & — & — & — \\ 
            FLIR aligned \cite{zhang2020multispectral} & 5k\phantom{.0} & 3 & \checkmark & — & 640 $\times$ 512 & 640 $\times$ 512 & — & \checkmark & — & — & — \\
            
            %\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
            
            \phantom{LYNRED} MD (ours) & 4k\phantom{.0} & 9 & \checkmark & — & 640 $\times$ 480 & 1280 $\times$ 960 & — & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
            % \cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
        \end{tabular}
    }
    \caption{Datasets specifications for all the presented RGB-T datasets. We use ($^\star$) to signal that image size is variable. In this case, only the most frequent size is displayed.}
    \label{tab:datasetsspecs}
\end{table*}


\paragraph{Honorable mentions}

Among existing datasets, InfraParis~\cite{franchi2024infraparis} is the most similar in scope to ours, as it provides annotations for both infrared and RGB images acquired around Paris, France. However, due to significant differences in the fields of view between the two modalities, it is unsuitable for multispectral or multimodal object detection tasks. Another notable dataset is MFNet~\cite{takumi2017multispectral}, which offers both bounding box annotations and semantic segmentation masks for a variety of road users in urban environments in Tokyo, Japan. Lastly, the SJTU Multispectral Object Detection (SMOD) Dataset~\cite{chen2024amfd} focuses on scenes with a high density of vulnerable road users, particularly pedestrians and cyclists, making it well-suited for safety-critical perception research.








==> Parts/03_Datadesc.tex <==
\section{Dataset description}
\label{sec:dataset_description}

This dataset is---to the best of our knowledge---the first large--scale European ADAS dataset specifically focusing on VRU detection in multimodal infrared imagery. \phantom{LYNRED} MD consists of a total of 4,000 images, divided into 3,168 image pairs for training and 832 for testing. The data was collected in the surroundings of Grenoble (France). It includes a diverse range of driving scenarios from winter snowy ski resorts to summer sunny urban areas.\\[-.3cm]

Images were acquired all year round, covering a wide range of ambient temperatures from 3.7\si{\celsius} to 30\si{\celsius}. This temperature variability presents a significant challenge for thermal or long wave infrared (LWIR) sensors since they operate by capturing thermal radiation. When environmental temperatures approach that of the human body, the contrast between objects and their surroundings decreases, potentially affecting detection performance, see figure \ref{fig:temperaturecontrasts} for an example.\\[-.3cm]

\begin{figure*}[tbp]
    \centering
    \begin{subfigure}{ 0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/merged_hiver1.png}
        \caption{external temperature: \num{ 5.4}\si{\celsius}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{images/summerpic.png}
        \caption{external temperature: \num{30}\si{\celsius}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width= \linewidth]{images/summernight.png}
        \caption{external temperature: \num{20.6}\si{\celsius}}
    \end{subfigure}
    \caption{Images from a broad range of seasonal and heat scenarios are present in the \phantom{LYNRED} mobility dataset offering challenging conditions for developing infrared based AEB.}
    \label{fig:temperaturecontrasts}
\end{figure*}

To prevent data leakage, the sequences were split into separate training and testing subsets while ensuring a representative distribution of time of day and seasonal conditions. The distribution of the dataset split accross various parameters is featured in figure~\ref{fig:train-test-distrib}.\\[-.3cm] 


\begin{figure*}[!ht]
    \centering
    \begin{subfigure}{1\linewidth}
        \centering
        \includegraphics[trim=0 1cm 0 1cm, width=0.99\linewidth]{images/alltrain.png}
        \caption{Train dataset}
    \end{subfigure}
    \begin{subfigure}{0.99\linewidth}
        \centering
        \includegraphics[trim=0 1cm 0 .5cm, width=1\linewidth]{images/alltest.png}
        \caption{Test dataset}
    \end{subfigure}
    \caption{Decomposition of the different data splits.}
    \label{fig:train-test-distrib}

\end{figure*}

Additionally, 9 different classes are annotated to reflect the diversity of road users. A comprehensive comparison of class labels across the existing datasets' training sets is presented in Table~\ref{tab:classimbalance}. We chose to annotate fewer classes to counteract the class imbalance. As a matter of fact, 6 out of the 16 classes of FLIR have under 100 samples in the train set and most of these are not present in the test set~\cite{FLIR}. Furthermore, the occlusion status of human--class objects is also recorded, following the method used in other existing infrared object detection datasets~\cite{FLIR, jia2021llvip, chen2024amfd}.\\[-.3cm]

\begin{table*}[!h]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{cccccccccccccccc}
        \hline
        \multirow{Datasets} & \multicolumn{15}{c}{Number of instances per class}    \\ 
         &  person & bicycle &  car &  motorcycle &  bus &   train &   truck &   light &   hydrant &   sign &   Animal  &   skateboard &    stroller &    scooter &  other vehicle \\ \hline
         
         
           KAIST \cite{hwang2015multispectral} &   \num{103128} &   - &   - &  - &   - &   - &   - &   - &   - &   - &   - &    - &   - &   -   &  - \\ 
         
         
                FLIR ADAS \cite{FLIR} &   \num{50478} &  \num{7237}  & \num{73623}  & \num{1116} & \num{2245} & \num{5} &  \num{829} & \num{16198} & \num{1095}  &  \num{20770} & \num{12} $\star$ & \num{29}  &  \num{15}  &  \num{15}    & \num{1373}  \\ 
         
         
                LLVIP \cite{jia2021llvip} &  34137  &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &    -   &  -  \\ 
         
         
                M3FD \cite{m3fd} &  7443  &   - &  11737 &  344   &  449  &  - &  654  & 1542  &   - &   - &   - &   - &   - &   -   &  -  \\ 
         
         
                KAIST sanitized \cite{chen2024amfd} & 24247  &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &   - &   -   &  -  \\ 
         
         
                FLIR aligned \cite{zhang2020multispectral} & 8987 & 2566 & 20608 &   - &   - &   - &   - &   - &   - &   - &    - &   - &   - &   -   &  -  \\ 
         
         
                \phantom{LYNRED} MD (ours) &  9794 & 1794  & 17411 &  350  &  249  &   330 &   530 &   - &   - &   - &   106 & - &   - &   -   &  91   \\ \hline
        \end{tabular}
    }
    \caption{Number of instances per class across the different reference  RGB-T datasets. The number of annotations displayed corresponds to the infrared train split. We notice that even though FLIR offers far more classes than others, the class imbalance makes most of those useless for training. The Starred $\star$ value represents blended classes (4 dogs and 8 deers).}
    \label{tab:classimbalance}
\end{table*}

We provide both 14 bits per pixels and processed 8 bits per pixels infrared images, as tone mapping has been shown to be a relevant component of the embedded object detection pipeline~\cite{karam2024optimizing}. The 14bit images correspond to the minimally processed output of the infrared camera. The amount of processing applied was determined using the work from Karam \etal~\cite{karam2024optimizing}.\\[-.3cm]

\begin{figure*}[!htbp]
   \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=1 \linewidth]{images/OURS_ALL.png}
        \caption{}
        \label{fig:Cumulative_all}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/OURSVSFLIR_ALL.png}
        \caption{}
        \label{fig:Cumulative_FLIRvs}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/OURDATSET_FINAL.png}
        \caption{}
    \end{subfigure}
    \caption{Cumulative histograms of bounding boxes height for all presented datasets (a), comparison between FLIR ADAS, FLIR Aligned and \phantom{LYNRED} MD IR splits (b)  and \phantom{LYNRED} MD's RGB and IR modalities (c). The gap between IR and RGB annotation sizes for curve (c) can be explained by the difference between the IR and RGB sensors specifications.}
    \label{fig:Cumulative}
\end{figure*}

In figure \ref{fig:Cumulative} we plot the empirical cumulative density of bounding box height for each dataset, this allows to pinpoint some important differences between the datasets concerning object size annotations. We can clearly see that our dataset is on par with most other RGB-T datasets resembling M3FD the most with respect to its bounding box height distribution. The task shift between LLVIP and others is easily remarkable, as objects in video surveillance clips are at a controlled distance from the camera,  leading to a smaller variance and overall bigger boxes.\\[-.3cm]

Finally, in the multimodal detection subset of \phantom{LYNRED}-MD objects as small as 4 pixels in height are annotated. This is done to evaluate the efficiency of infrared sensors for pedestrian detection in the context of regulatory standards cited in the introduction~\cite{NHTSA}. To assess the capability of detecting pedestrians at a distance of 50 meters, we estimate the expected pixel height $h_{\text{object}}$ of an unobstructed human in our dataset by $h_{\text{object}} = \frac{f \times H_{\text{object}} \times h_{\text{image}}}{D_{\text{object}}\times H_{\text{sensor}}}$ derived from~\cite{szeliski2022computer} and where $H_x$ and $h_x$ refer to physical height (mm) or height in pixels, respectively.\\[-.3cm]

For an average adult pedestrian height provided by NHTSA as $H_{\text{object}} = 1.750\si{\meter}$~\cite{NHTSAheight} and in order to meet regulatory requirements with our sensor setup specifications, we compute a necessity to detect objects with a minimum height of approximately 24.1 pixels on the ATTO sensor (focal length $f = 14\si{\milli\meter}$, image height $h_{\text{image}} = 480\text{ pixels}$, sensor height $H_{\text{sensor}} = 8.16\si{\milli\meter}$, object distance $d_{\text{object}} = 50\si{\meter}$), respectively 34.1 pixels for the PICO sensor (sensor height $H_{\text{sensor}} = 5.76\,\text{mm}$).\\[-.3cm]

Applying the same calculation to FLIR’s dataset yields a comparable value of 20.9 pixels. We also performed the computation for a child--sized pedestrian (approximately 100\si{\cenit\meter} tall), which establishes more challenging detection threshold of 13.8 and 19.5 pixels for the ATTO and the PICO sensors, respectively. Meanwhile they would be 11.9 pixels in FLIR's dataset.\\[-.3cm]

In Figure~\ref{fig:Cumulative_FLIRvs}, we illustrate the pixel height thresholds for all unobstructed pedestrian annotations in the FLIR ADAS validation set, as well as the FLIR Aligned and \phantom{LYNRED} MD test datasets. Notably, in both datasets, nearly 40\% of annotated humans are 29 pixels tall or smaller. These datasets thus provide a strong benchmark for testing AEB systems, especially in critical situations where detecting small objects remains a significant challenge for object detection algorithms~\cite{gundougan2023ir, li2021yolo,wei2024review}.\\[-.3cm]

Images were anonymised using the blurring algorithm from~\cite{anonymizer} targetting licence plates and faces to make the dataset compliant with the regulations of the CNIL (\emph{Commission Nationale de l’Informatique et des Libertés}), the French data protection authority.


==> Parts/04_experiments.tex <==
\section{Benchmark}
\label{sec:benchmark}

To benchmark our dataset, we evaluated the finetuning performances of YOLOv8n~\cite{Jocher_Ultralytics_YOLO_2023}, pretrained on the COCO dataset~\cite{lin2014microsoft}. We selected this model for its ease of use and suitability for deployment. The model is fine-tuned for 200 epochs with a batch size of 16, using the "auto" optimizer setting provided by Ultralytics. \\[-.3cm]


Rather than focusing solely on in-domain performances, our work emphasizes on the model's generalization capabilities. To assess this, we adopted mAP@50 (mean Average Precision at an Intersection-over-Union threshold of 0.5) as our evaluation metric. This threshold is commonly used in object detection benchmarks and offers a reasonable balance between detection quality and tolerance for localization error particularly important when detecting small or low-contrasted objects in thermal imagery.\\[-.3cm]

\begin{table}[!ht]
  \centering
  \begin{subfigure}{0.49\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{|c|cccccc|}
            \cline{2-7}
            \multicolumn{1}{l|}{} & \multicolumn{6}{c|}{Train dataset} \\
            \hline
              Test dataset & ALL & LLVIP & FLIR & FLIR Aligned & M3FD & \textbf{ours}\\
            \hline
              ALL & \cellcolor{gray!60}  \textbf{0.89} & 0.61 & 0.53 & 0.54 & 0.58 & \cellcolor{gray!30}  0.74 \\

              LLVIP & \cellcolor{gray!60}  \textbf{0.96} & \cellcolor{gray!60}  \textbf{0.96} & 0.41 & 0.44 & 0.64 & \cellcolor{gray!30}  0.81 \\
                
              FLIR ADAS & 0.60 & 0.11 & \cellcolor{gray!60}  \textbf{0.80} & 0.55  & 0.43 & \cellcolor{gray!30}  0.62 \\
              
              FLIR Aligned & \cellcolor{gray!60}  \textbf{0.85} & 0.22 & 0.79 & \cellcolor{gray!30}  0.81 & 0.48 & 0.76 \\
              
              M3FD & \cellcolor{gray!60}  \textbf{0.86} & 0.29 & \cellcolor{gray!30}  0.67 & 0.54 & \cellcolor{gray!60}  \textbf{0.86} & 0.62 \\
              
              \textbf{ours} & \cellcolor{gray!60}  \textbf{0.62} & 0.17 & 0.45 & 0.41 & 0.32 & \cellcolor{gray!30}  0.57 \\
             \hline 
        \end{tabular}
        }
        \caption{IR}
        \label{tab:map50_humanIR}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
         \begin{tabular}{|c|cccccc|}
            \cline{2-7}
            \multicolumn{1}{l|}{} & \multicolumn{6}{c|}{Train dataset} \\
            \hline
            Test dataset & ALL & LLVIP & FLIR & FLIR Aligned & M3FD & \textbf{ours} \\
            \hline
            ALL & \cellcolor{gray!60}  \textbf{0.57} & 0.37 & 0.23 & 0.24 & \cellcolor{gray!30}  0.38 & 0.35 \\
            LLVIP & \cellcolor{gray!60}  \textbf{0.63} & \cellcolor{gray!30}  0.54 & 0.17 & 0.11 & 0.36 & 0.31 \\
            
            FLIR ADAS & 0.39 & 0.14 & \cellcolor{gray!60}  \textbf{0.70} & 0.39 & 0.39 & \cellcolor{gray!30}  0.49 \\
            
            FLIR Aligned & \cellcolor{gray!60}  \textbf{0.88} & 0.24 & 0.58 &\cellcolor{gray!30}  0.64 & 0.51 & 0.48 \\
            
            M3FD & \cellcolor{gray!60}  \textbf{0.73} & 0.23 & 0.42 & 0.24 & \cellcolor{gray!30}  0.77 & 0.37 \\
            
            \textbf{ours} & \cellcolor{gray!60}  \textbf{0.61} & 0.06 & 0.35 & 0.19 & 0.21 & \cellcolor{gray!30} 0.49 \\
            \hline
        \end{tabular}
        }
        \caption{RGB}
        \label{tab:map50_humanRGB}
    \end{subfigure}
  \caption{Mean Average Precision (mAP@50) for human detection across~\subref{tab:map50_humanIR} IR and~\subref{tab:map50_humanRGB} RGB datasets. Only the 'person' class is retained for comparison purposes. Each column uses a same training dataset and each row uses a same evaluation dataset. The "ALL" dataset combines LLVIP, FLIR Aligned, M3FD, and ours. All experiments were conducted using YOLOv8n trained for 200 epochs. The best result per column is highlighted in bold and dark gray; the second best is highlighted in light gray.}
  \label{tab:map50_human}
\end{table}

Our generalization test protocol involves training the model on one dataset and evaluating it on the others. We focus exclusively on the "person" or "human" class, as it is the most relevant for VRU detection tasks. The datasets used in our experiments are FLIR ADAS, FLIR Aligned, M3FD, LLVIP, and ours. Additionally, we include a combined dataset, referred to as ALL, which merges LLVIP, FLIR Aligned, M3FD, and ours. This serves as a topline reference. The comparative results across datasets are presented in Table~\ref{tab:map50_human}.\\[-.3cm]

Table~\ref{tab:map50_human} highlights several key findings. First, the model trained on the "ALL" dataset achieves the best performance on its constituent datasets LLVIP, FLIR Aligned, M3FD, and ours. In contrast, performance on FLIR ADAS - excluded from the "ALL" set - is notably lower. This, as well as FLIR Aligned's performance on FLIR ADAS's test set suggests that FLIR Aligned may not fully capture the data distribution of the broader FLIR ADAS dataset.\\[-.3cm]

Second, we observe a modality gap: IR generally outperform RGB across datasets in object detection. This trend is especially pronounced in datasets such as LLVIP, which focuses on nighttime or low-light conditions where RGB sensors are less effective. Interestingly, despite LLVIP's size being far larger than most other datasets, its models perform poorly in cross--dataset validation. This emphasizes the relevance of task specific datasets focussing on driving scenarios.\\[-.3cm]

Our dataset stands out both in difficulty and generalization potential. The model trained on our IR images achieve the second-best performance on three out of the five datasets (excluding FLIR ADAS for FLIR Aligned). Furthermore, the multimodal subset of \phantom{LYNRED} MD consistently proves challenging for models trained on other driving-related datasets, often ranking as the most difficult test set. These findings support the claim that \phantom{LYNRED} MD introduces a new level of challenge for infrared-based pedestrian detection and is a valuable benchmark for future AEB system development.









==> Parts/05_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


In this paper, we introduced the multimodal detection subset of the \phantom{LYNRED} Mobility Dataset, comprised of 4000 RGB--IR image pairs captured under diverse weather, lighting, and road  conditions  around  Grenoble,  France. To our knowledge, this dataset is the only RGB-T data set adressing challenging meteorological situations. This is of critical importance and a clear improvement with respect to existing data sets because these adversarial situations are precisely the ones where most casualities happen and where advanced driver assistance systems can actually make a real difference.  Our  dataset  spans  varied  driving  contexts (urban, rural, mountainous, etc.)  and a vehicle fleet compliant with Western European standards. We show that models trained on our dataset achieve improved generalization and transfer performance on Yolov8n benchmarks.  Compared to others it remains performant on any proposed IR pedestrian detection task, whether surveillance or more closely related to pedestrian detection. In the future we expect to expand the dataset and provide a geometrically aligned version of the RGB modality. This will allow the development of multispectral object detection which was not studied in this paper. We also wish to expand our study method to more datasets and models such as MFNet or SMOD datasets. Alongside this dataset we also release the stereovision and Range Estimation subsets of the \phantom{LYNRED} mobility dataset. We hope these will help to promote and spread the use of infrared sensors.


==> Parts/_abstract.tex <==
Current road safety systems primarily focus on minimizing post-collision damage. However, advances in algorithmic perception are shifting focus toward early collision prediction, especially in low-visibility conditions like nighttime or fog, where thermal infrared sensing outperforms both human vision and RGB imaging. While available RGB-infrared datasets such as FLIR ADAS and LLVIP are good benchmarks, they mostly consists of clear weather and overly simple scenarios. In this paper, we introduce the LYNRED MD Multimodal Detection Dataset, a subset of the LYNRED Mobility Dataset, comprised of \num{4000} RGB-infrared image pairs captured under diverse weather, lighting, and road conditions around Grenoble, France. Our dataset spans varied driving contexts (urban, rural, mountainous, etc.) and a vehicle fleet compliant with Western European standards. We show that models trained on our dataset achieve improved generalization and transfer learning performance on a Yolov8 benchmark. By covering critical edge cases, our dataset supports the development of more reliable and deployable vision systems for advanced driver-assistance systems.




